CAD-VAE: Leveraging Correlation-Aware Latents for Comprehensive Fair Disentanglement

While deep generative models have significantly advanced representation learning, they may inherit or amplify biases and fairness issues by encoding sensitive attributes alongside predictive features. Enforcing strict independence in disentanglement is often unrealistic when target and sensitive factors are naturally correlated. To address this challenge, we propose \textbf{CAD-VAE} (\textbf{C}orrelation-\textbf{A}ware \textbf{D}isentangled \textbf{VAE}), which introduces a correlated latent code to capture the information shared between the target and sensitive attributes. Given this correlated latent, our method effectively separates overlapping factors without extra domain knowledge by directly minimizing the conditional mutual information between target and sensitive codes. A relevance-driven optimization strategy refines the correlated code by efficiently capturing essential correlated features and eliminating redundancy. Extensive experiments on benchmark datasets demonstrate that CAD-VAE produces fairer representations, realistic counterfactuals, and improved fairness-aware image editing. Source code is available : https://github.com/merry7cherry/CAD-VAE

==> tables/reb_ablation.tex <==
\begin{table}[h]
\vspace{-1em}
\centering
% \caption{Ablation Study}
\label{tb:quantitative_edit}
\renewcommand{\arraystretch}{0.85} % 更紧凑的行距
\setlength{\tabcolsep}{2pt}       % 更紧凑的列间距
\begin{adjustbox}{width=0.95\columnwidth,center}
\begin{tabular}{c||ccc|ccc} 
\Xhline{2\arrayrulewidth}
\rowcolor{gray!20}
\textbf{Setting} & \multicolumn{3}{c|}{CelebA} & \multicolumn{3}{c}{Color bias MNIST}\\ 
\rowcolor{gray!20}  
& Acc $\uparrow$ & EOD $\downarrow$ & DP $\downarrow$ & Acc $\uparrow$ & EOD $\downarrow$ & DP $\downarrow$ \\
\hline
$w/o \ \mathcal{L}_{\text{CMI}}$ & 0.948 & 0.188 & 0.212 & 0.989 & 0.208 & 0.245  \\ 
$w/o \ \mathcal{L}_{\text{LRI}}$ & 0.909 & 0.057 & 0.156 & 0.942 & 0.096 & 0.204  \\ 
$w/o \ \mathcal{L}_{\text{TC}}$  & 0.928 & 0.067 & 0.164 & 0.981 & 0.132 & 0.174  \\ 
\textbf{Ours}  & \textbf{0.923} & \textbf{0.021} & \textbf{0.112} & \textbf{0.977} & \textbf{0.076} & \textbf{0.118} \\
\hline
iVAE [2] & 0.887 & 0.096 & 0.121 & 0.953 & 0.127 & 0.148 \\ 
\hline
\end{tabular}
\end{adjustbox}
\vspace{-1.0em}
\end{table}


==> tables/reb_iVAE.tex <==
\begin{table}[h]
\vspace{-1em}
\centering
% \caption{Ablation Study}
\label{tb:quantitative_edit}
\renewcommand{\arraystretch}{0.9} % 调整行距
\setlength{\tabcolsep}{3pt} % 调整列间距
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{c||cccccc} 
\Xhline{2\arrayrulewidth}
\rowcolor{gray!20}
\textbf{Setting} & \multicolumn{3}{c|}{CelebA} & \multicolumn{3}{c|}{Color bias MNIST}\\ 
\rowcolor{gray!20}  
& Acc $\uparrow$ & EOD $\downarrow$ & DP $\downarrow$ & Acc $\uparrow$ & EOD $\downarrow$ & DP $\downarrow$ \\
\hline
$w/o \ \mathcal{L}_{\text{CMI}}$ & 0.948 & 0.188 & 0.212 & 0.989 & 0.208 & 0.245  \\ 
\hline
$w/o \ \mathcal{L}_{\text{LRI}}$ & 0.909 & 0.057 & 0.156 & 0.942 & 0.096 & 0.204  \\ 
\hline
$w/o \ \mathcal{L}_{\text{TC}}$ & 0.928 & 0.067 & 0.164 & 0.981 & 0.132 & 0.174  \\ 
\hline
Ours & \textbf{0.923} & \textbf{0.021} & \textbf{0.112} & \textbf{0.977} & \textbf{0.076} & \textbf{0.118} \\ 
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{adjustbox}
\vspace{-1.0em}
\end{table}
